Convergence and Applications of ADMM on the Multi-convex Problems

In recent years, although the Alternating Direction Method of Multipliers (ADMM) has been empirically applied widely to many multi-convex applications, delivering an impressive performance in areas such as nonnegative matrix factorization and sparse dictionary learning, there remains a dearth of generic work on proposed ADMM with a convergence guarantee under mild conditions. In this paper, we propose a generic ADMM framework with multiple coupled variables in both objective and constraints. Convergence to a Nash point is proven with a sublinear convergence rate $o(1/k)$. Two important applications are discussed as special cases under our proposed ADMM framework. Extensive experiments on ten real-world datasets demonstrate the proposed framework's effectiveness, scalability, and convergence properties. We have released our code at \url{https://github.com/xianggebenben/miADMM}.

==> defs.tex <==

% Counter for keeping track of comments
\newcounter{revcomcounter}

% Command for reading the review comment counter
\renewcommand{\therevcomcounter}{\arabic{revcomcounter}}

% Review comment environment
\newenvironment{revcom}[1][]{%
\refstepcounter{revcomcounter}%
\ifx\\#1\\%
\else
\label{#1}%
\fi
\begin{trivlist}\item\textbf{Comment~\therevcomcounter: }\em%
}%
{\end{trivlist}}%

% Environment for responding to review comments
\newenvironment{response}[1][]{%
\begin{trivlist}\item\textbf{Response: }%
}%
{\end{trivlist}}%

